MTVNet: Mapping using Transformers for Volumes -- Network for Super-Resolution with Long-Range Interactions

Until now, it has been difficult for volumetric super-resolution to utilize the recent advances in transformer-based models seen in 2D super-resolution. The memory required for self-attention in 3D volumes limits the receptive field. Therefore, long-range interactions are not used in 3D to the extent done in 2D and the strength of transformers is not realized. We propose a multi-scale transformer-based model based on hierarchical attention blocks combined with carrier tokens at multiple scales to overcome this. Here information from larger regions at coarse resolution is sequentially carried on to finer-resolution regions to predict the super-resolved image. Using transformer layers at each resolution, our coarse-to-fine modeling limits the number of tokens at each scale and enables attention over larger regions than what has previously been possible. We experimentally compare our method, MTVNet, against state-of-the-art volumetric super-resolution models on five 3D datasets demonstrating the advantage of an increased receptive field. This advantage is especially pronounced for images that are larger than what is seen in popularly used 3D datasets. Our code is available at https://github.com/AugustHoeg/MTVNet

==> sec/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> sec/A1_suppl_2.tex <==
\clearpage
\setcounter{page}{1}
\maketitlesupplementary

\section{Details of SVHAT layer}



\begin{figure}[h]
   \centering
   %\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   \includegraphics[width=0.8\linewidth]{figs/svhat_overview_2_2.pdf}
   \caption{Overview of proposed SVHAT layer that captures global and local token dependencies using separate attention branches for CATs (\textcolor{red}{red}) and ITEs (\textcolor{blue}{blue}). The first branch follows the attention procedure from FasterViT \cite{Hatamizadeh_FasterViT}, whereas the second follows the approach from SwinV2 \cite{Liu_SwinV2}. We use CSM modules to merge tokens from preceding levels before computing attention in each branch.}
   \label{fig:svhat_layer}
\end{figure}

\section{Training details}

\subsection{Datasets}

\textbf{Human Connectome Project (HCP) 1200}\\ The HCP 1200 Subjects Data Release \cite{Van_HCP_1200_dataset} includes structural MRI scans from 1113 healthy subjects acquired using a 3T scanning platform. We use the T1-weighted images, featuring an isotropic resolution of 0.7 mm and a matrix size of $320\times320\times256$. Following \cite{Chen_mDCSRN_C, Forigua_SuperFormer}, the dataset is split into 780 subjects for training, and 111 each for validation, evaluation, and testing. Performance evaluation is conducted solely on the test set.

\textbf{Information eXtraction from Images (IXI)}\\ The IXI dataset contains multi-modality MRI data (PD-, T1-, and T2-weighted) from 600 healthy subjects scanned with one 3T and two 1.5T scanning platforms. We use 581 T1-weighted scans, of which 507 have a resolution of $0.9375\times0.9375\times1.2$ mm and a matrix size of $256\times256\times150$, while the remaining 74 have a similar resolution but a matrix size of $256\times256\times146$. The dataset is split into 500 subjects for training, 6 for validation, and 75 for testing, with evaluation performed on the test set.

\textbf{Brain Tumor Segmentation Challenge (BraTS) 2023}\\ For BraTS 2023, we use 1470 T1-weighted skull-stripped MRI scans of glioma patients, standardized to an isotropic resolution of 1 mm and a matrix size of $240\times240\times155$. The provided dataset split allocates 1251 subjects for training and 219 for validation, with evaluation performed on the validation set.

\textbf{Kirby 21}\\ The Kirby 21 dataset includes multi-modality MRI scans from healthy individuals with no history of neurological conditions. We use the 42 T2-weighted images, which have a resolution of $1\times0.9375\times0.9375$ mm and a matrix size of $180\times256\times256$. The data is split into 37 images for training (KKI-06 to KKI-42) and 5 for testing (KKI-01 to KKI-05).

\textbf{Femur Archaeological CT Superresolution (FACTS)}\\ The FACTS dataset comprises 12 archaeological proximal femurs scanned with clinical-CT and micro-CT platforms \cite{Bardenfleth_FACTS}. Clinical-CT scans have a resolution of $0.21\times0.21\times0.4$ mm, while micro-CT scans have a resolution of $58\times58\times58$ $\mu$m. Clinical-CT volumes are registered and linearly interpolated to match the micro-CT matrix size. The dataset is split into 10 images for training and 2 (f\_002 and f\_138) for testing.

\begin{figure}[t]
    \centering
        \begin{subfigure}{\linewidth}
        \includegraphics[width=1.0\linewidth]{figs/visual_comparisons/LAM_FACTS_Synth_4x_cube_003.png}
        %\caption{LAM comparison of SR models from FACTS-Synth at $4 \times$ upscaling.}
        %\label{fig:LAM_visualisation}
        \end{subfigure}
        \begin{subfigure}{\linewidth}
        \includegraphics[width=1.0\linewidth]{figs/visual_comparisons/LAM_FACTS_Synth_4x_cube_002.png}
        %\caption{LAM comparison of SR models from FACTS-Synth at $4 \times$ upscaling.}
        %\label{fig:LAM_visualisation}
        \end{subfigure}
        \begin{subfigure}{\linewidth}
        \includegraphics[width=1.0\linewidth]{figs/visual_comparisons/LAM_FACTS_Synth_4x_03.png}
        %\caption{LAM comparison of SR models from FACTS-Synth at $4 \times$ upscaling.}
        %\label{fig:LAM_visualisation}
        \end{subfigure}
        \caption{LAM comparisons of SR models using FACTS-Synth at $4 \times$ upscaling.}
        \label{fig:LAM_comparisons_supp}
\end{figure}

\section{Visual comparisons using LAM}

The hierarchical architecture of \networkname should ideally help the network take advantage of more surrounding pixels when predicting the SR image. To verify this, we use the LAM attribution method \citep{gu2021interpreting} to analyze the influence of the input pixels on the SR output. The LAM method is a modification of the integrated gradient method \citep{sundararajan2017axiomatic}, specifically designed to investigate SR architectures. It works by accumulating the gradient over interpolations between the input and a blurred version of the input. We have modified the method for 3D analysis and we show the LAM results for all seven model architectures in \cref{fig:LAM_visualisation} for a selected area of a slice and also report the diffusion index (DI), which is a measure of the range of pixels involved in the predicted SR output.


\begin{comment}
\begin{figure*}[h]
  \centering
  \begin{subfigure}{0.49\linewidth}
    \includegraphics[width=1.0\linewidth]{figs/visual_comparisons/SR_comparison_HCP_1200_4x_no_metrics_2_T.png}
    %\caption{Subfigure 1.}
    %\label{fig:subfig1}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.49\linewidth}
    \includegraphics[width=1.0\linewidth]{figs/visual_comparisons/SR_comparison_IXI_4x_no_metrics_2_T.png}
    %\caption{Subfigure 2.}
    %\label{fig:subfig2}
  \end{subfigure}
  
  \vspace{0.5em} % Space between the rows

  \begin{subfigure}{0.49\linewidth}
    \includegraphics[width=1.0\linewidth]{figs/visual_comparisons/SR_comparison_FACTS_Synth_4x_no_metrics_2_T.png}
    %\caption{Subfigure 3.}
    %\label{fig:subfig3}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.49\linewidth}
    \includegraphics[width=1.0\linewidth]{figs/visual_comparisons/SR_comparison_FACTS_Real_4x_no_metrics_2_T.png}
    %\caption{Subfigure 4.}
    %\label{fig:subfig4}
  \end{subfigure}
  %\vspace{-0.5em} % Space between the rows
  \caption{Visual comparisons of SR model outputs from the datasets HCP 1200, IXI, FACTS-Synth, and FACTS-Real using $4\times$ upscaling. The ground truth (GT) and LR input images are shown side-by-side in the top-left separated by the red line.}
  \label{fig:visual_comparison}
\end{figure*}
\end{comment}


%\section{Complexity analysis of \networkname}

\section{More visual comparisons}



\begin{figure*}[h]
  \centering
  \begin{subfigure}{0.49\linewidth}
    \includegraphics[width=1.0\linewidth]{figs/visual_comparisons/SR_comparison_FACTS_Synth_4x_no_metrics_2_T_supp.png}
    %\caption{Subfigure 1.}
    %\label{fig:subfig1}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.49\linewidth}
    \includegraphics[width=1.0\linewidth]{figs/visual_comparisons/SR_comparison_FACTS_Real_4x_no_metrics_2_T_supp.png}
    %\caption{Subfigure 2.}
    %\label{fig:subfig2}
  \end{subfigure}
  
  \vspace{0.5em} % Space between the rows

  \begin{subfigure}{0.49\linewidth}
    \includegraphics[width=1.0\linewidth]{figs/visual_comparisons/SR_comparison_HCP_1200_4x_no_metrics_2_T_supp.png}
    %\caption{Subfigure 3.}
    %\label{fig:subfig3}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.49\linewidth}
    \includegraphics[width=1.0\linewidth]{figs/visual_comparisons/SR_comparison_IXI_4x_no_metrics_2_T_supp.png}
    %\caption{Subfigure 4.}
    %\label{fig:subfig4}
  \end{subfigure}

  \vspace{0.5em} % Space between the rows

  \begin{subfigure}{0.49\linewidth}
    \includegraphics[width=1.0\linewidth]{figs/visual_comparisons/SR_comparison_BRATS2023_4x_no_metrics_2_T.png}
    %\caption{Subfigure 3.}
    %\label{fig:subfig3}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.49\linewidth}
    \includegraphics[width=1.0\linewidth]{figs/visual_comparisons/SR_comparison_KIRBY21_4x_no_metrics_2_T.png}
    %\caption{Subfigure 4.}
    %\label{fig:subfig4}
  \end{subfigure}
  %\vspace{-0.5em} % Space between the rows
  \caption{Visual comparisons of SR model outputs from the datasets HCP 1200, IXI, FACTS-Synth, and FACTS-Real using $4\times$ upscaling. The ground truth (GT) and LR input images are shown side-by-side in the top-left separated by the red line.}
  \label{fig:visual_comparison}
\end{figure*}




\iffalse
\section{Rationale}
\label{sec:rationale}
% 
Having the supplementary compiled together with the main paper means that:
% 
\begin{itemize}
\item The supplementary can back-reference sections of the main paper, for example, we can refer to \cref{sec:intro};
\item The main paper can forward reference sub-sections within the supplementary explicitly (e.g. referring to a particular experiment); 
\item When submitted to arXiv, the supplementary will already included at the end of the paper.
\end{itemize}
% 
To split the supplementary pages from the main paper, you can use \href{https://support.apple.com/en-ca/guide/preview/prvw11793/mac#:~:text=Delete%20a%20page%20from%20a,or%20choose%20Edit%20%3E%20Delete).}{Preview (on macOS)}, \href{https://www.adobe.com/acrobat/how-to/delete-pages-from-pdf.html#:~:text=Choose%20%E2%80%9CTools%E2%80%9D%20%3E%20%E2%80%9COrganize,or%20pages%20from%20the%20file.}{Adobe Acrobat} (on all OSs), as well as \href{https://superuser.com/questions/517986/is-it-possible-to-delete-some-pages-of-a-pdf-document}{command line tools}.
\fi

